On the convergence of policy gradient methods to Nash equilibria in general stochastic games

Learning in stochastic games is a notoriously difficult problem because, in addition to each other's strategic decisions, the players must also contend with the fact that the game itself evolves over time, possibly in a very complicated manner. Because of this, the convergence properties of popular learning algorithms - like policy gradient and its variants - are poorly understood, except in specific classes of games (such as potential or two-player, zero-sum games). In view of this, we examine the long-run behavior of policy gradient methods with respect to Nash equilibrium policies that are second-order stationary (SOS) in a sense similar to the type of sufficiency conditions used in optimization. Our first result is that SOS policies are locally attracting with high probability, and we show that policy gradient trajectories with gradient estimates provided by the REINFORCE algorithm achieve an $\mathcal{O}(1/\sqrt{n})$ distance-squared convergence rate if the method's step-size is chosen appropriately. Subsequently, specializing to the class of deterministic Nash policies, we show that this rate can be improved dramatically and, in fact, policy gradient methods converge within a finite number of iterations in that case.

==> App-Contents.tex <==
%----------------------------------------------------------------------
%%% APP: CONTENTS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


%The remainder of this paper is organized as follows. In \cref{app:organization}, we list a glossary of all the basic concepts and notation that we will utilize throughout the paper.
%In \cref{app:errata}, we expand the discussion for the related work in general-sum stochastic games and we describe all the typos and corrections in definitions or statements between the submission of main part and supplementary.
%In \cref{app:marl}, we prove all the properties of the Markov Decision Process (MDP), the value function and its gradient for the multi-agent reinforcement learning process when the model of episodic random stopping is in run. While similar machinery have been considered for the infinite horizon with $\gamma$ discounting regime and a standard analogy has been described in the literature, we prove here explicitly for the sake of completeness.
%In \cref{app:solutions}, we consider the different optimization solutions from variational perspective and their connection to Markov stationary Policy Nash Equilibria.
%In \cref{app:reinforce}, we conclude our preliminary results with the statistical guarantees of \reinforce policy gradient estimator.
%Finally, in \cref{app:asymptotic} we present the asymptotic convergence results for the variational stable points and\AG{I wrote we show  sos only for eager} establish the convergence rates for the ``eager'' and ``lazy'' stochastic policy gradient method for the second-order stationary points (See \cref{app:SOS}) and their deterministic counterparts (See \cref{app:deterministic}).

\begin{table}[tbp]
\label{tab:index}
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cp{12cm}}
\toprule
\textsc{Notation}
	&\textsc{Description}
	\\ % <-- added & and content for each column
\midrule
$\rstate\in\states$
	&States of the game
	\\
$\pure_\play\in\pures_\play$
	& Actions of agent $\play\in\players$
	\\
%		\hline
$\traj$
	&Episode trajectory
	\\
%		\hline
$\stopTime(\traj)$
	&Episode stopping time
	\\
%		\hline
$\stopPr$
	&Minimum stopping probability
	\\
%		\hline
$\realReward_{\play,\time}$
	&Realized reward of $\play$-th player at time $\time$
	\\
%		\hline
$\curr[\step]$
	&Step size at episode $\run$
	\\
%		\hline
$\expar_\run$
	&Explicit exploration parameter at episode $\run$
	\\
%		\hline
$\gvalue(\curr)$
	&Policy gradients at policy $\curr$ of episode $\run$
%	When we write $\gvalue_{\play,\pure_\play,\rstate}(\policy)$, we refer to the gradient value of agent $\play\in\players$ for the specific pure action $\pure_\play\in\pures_\play$ and state $\rstate\in\states$ evaluated in the policy $\policy$.
	\\
%		\hline
$\signal_\run$
	&Policy gradient proxy at episode $\run$.
%	We use the same notation with $\gvalue_\run(\policy)$
	\\
%		\hline
%$\dstate_\run$
%	&Aggregate gradients at round $\run$
%	\\
\bottomrule
\end{tabular}
\caption{Refresher of the most common notations used in our paper.}
\end{table}

==> App-Errata.tex <==
%----------------------------------------------------------------------
%%% APP: ERRATA
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


When preparing the supplementary material of our paper, we noticed a number of typographic errors and omissions in the main paper that could possibly cause confusion.
We clarify those below:
\begin{itemize}
\item
L48:
The reference pointers should point to \citet{Per13} and \citet{LPX20}.
\item
L157:
\eqref{eq:NP} should read \eqref{eq:FOS}
\item
L166:
Only the one-way implication is relevant;
\cref{prop:var} was amended accordingly.
\item
L188:
The text should read $\curr[\step] = \step/(\run + \runoff)^{\pexp}$ for some $\step>0$, $\runoff\geq0$ and $\pexp\geq0$.
\item
L246:
The text of \cref{thm:stable} was amended to explicitly include the above clarification.
\item
L251\textendash L252:
the relation ``$1-\pexp<\rexp/2<\pexp-1/2$'' should read ``$1-\pexp < \rexp < 2\pexp-1$''.
% The statement of \cref{cor:stable} has been amended to reflect this change.
%\item
%Corollary 1: Take cases for Model 1\&2 and Model 3
% \item
% Maybe change $\expar_\run = \expar/\run^{\rexp}$ to $\expar_\run = \expar/(\run+\runoff)^\rexp$ in all Corollaries
% \PM{Whatever you think looks best / simpler!}
% %\item
% %Theorem 1: We added $\step_\run$ in the statement, and also this about ``(or $\runoff$ large enough)''. 
% \item
% Corollary 1: Change $\step_\run = \step/\run^{\pexp}$ to $\step_\run = \step/(\run+\runoff)^{\pexp}$, and also decide whether we will include the ``$+\runoff$'' in the $\expar_\run$ definition (in all the Corollaries).
% \PM{Whatever you think looks best!}
\item L250, L283:
``$\curr[\mix] = \mix/\run^{\rexp}$'' should read  ``$\curr[\mix] = \mix/(\run+\runoff)^{\rexp}$'' and ``$\curr[\mix] = \mix/(\run+\runoff)^{\pexp/2}$'' respectively.
\item
L331, \cref{eq:lazy}:
``$\nhd$'' should read ``$\dbasin$''
\item L125, the \st{minimax} \emph{mismatch coefficient} can be defined either as $\mismatch\defeq\max_{\policy,\policy'\in\policies}\braces[\big]{\supnorm{\visitMeas{\stateDist}{\policy}/\visitMeas{\stateDist}{\policy'}} }$ or, more simply, as $\mismatch\defeq\max_{\policy,\in\policies}\braces[\big]{\tfrac{1}{\stopPr}\supnorm{\visitDistr{\stateDist}{\policy}/\stateDist} }$.

\end{itemize}
The errata and omissions identified above have all been corrected in the file at hand.

==> App-Test.tex <==
%----------------------------------------------------------------------
%%% APP: TEST
%----------------------------------------------------------------------
% !TEX root = ./Main.tex



\begin{example}
\label{ex:test}
This is a test example within a test appendix with a test equation:
\begin{subequations}
\begin{align}
\label{eq:test}
\new
	= \proxof{\point}{\dvec}
	&\iff
\new[\dpoint]
	= \dpoint + \dvec
	\quad
	\text{and}
	\quad
\new
	= \mirror(\new[\dpoint])
\shortintertext{where}
\dpoint
	\in \subd\hreg(\point)
	&\iff
\point
	\gets \mirror(\dpoint).
\end{align}
\end{subequations}
The first equation above can be referred as \eqref{eq:test}.
This concludes our example.
\endenv
\end{example}

The above example will be referred to as \cref{ex:test}.
